Protein as a Second Language for LLMs

Deciphering the function of unseen protein sequences is a fundamental challenge with broad scientific impact, yet most existing methods depend on task-specific adapters or large-scale supervised fine-tuning. We introduce the "Protein-as-Second-Language" framework, which reformulates amino-acid sequences as sentences in a novel symbolic language that large language models can interpret through contextual exemplars. Our approach adaptively constructs sequence-question-answer triples that reveal functional cues in a zero-shot setting, without any further training. To support this process, we curate a bilingual corpus of 79,926 protein-QA instances spanning attribute prediction, descriptive understanding, and extended reasoning. Empirically, our method delivers consistent gains across diverse open-source LLMs and GPT-4, achieving up to 17.2% ROUGE-L improvement (average +7%) and even surpassing fine-tuned protein-specific language models. These results highlight that generic LLMs, when guided with protein-as-language cues, can outperform domain-specialized models, offering a scalable pathway for protein understanding in foundation models.

==> table/dataset_example.tex <==
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{2pt}
\renewcommand\arraystretch{1.2}
    \centering\small
    \begin{tabular}{l|ccc|ccc|ccc}
\hline

\hline

\hline

\hline
        \multirow{2}{*}{\bf Model}& \multicolumn{3}{c|}{\bf ProtDescribe} & \multicolumn{3}{c|}{ \bf Protein2Text-QA}&\multicolumn{3}{c}{\bf Mol-Instructions}  \\
         & Dual & SeqOnly & QAOnly & Dual & SeqOnly & QAOnly & Dual & SeqOnly & QAOnly\\ 
\hline
        Qwen2.5-3B~\cite{qwen2.5} & 27.32 & 20.10 & 25.24 & 28.66 & 27.76 & 25.73 & 21.35 & 20.16 & 19.68 \\
        Mistral-7B-Instruct-v0.3~\cite{chaplot2023albert} & 29.39 & 19.46 & 25.24 & 28.59 & 21.85 & 22.68 & 19.12 & 14.31 & 17.40 \\
         Qwen3-14B~\cite{qwen3technicalreport} & 35.53 & 22.90 & 30.52 & 25.93 & 23.26 & 25.87 & 19.82 & 15.07 & 17.58\\
         kimi-k2~\cite{team2025kimi} & 35.91 & 28.58 & 32.43 & 21.04 & 17.10 & 18.06 & 15.54 & 12.79 & 12.09\\
         GPT-4o~\cite{openai2024gpt4} & 35.51 & 27.72 & 32.59 & 26.86 & 23.90 & 26.45 & 19.89 & 17.46 & 17.08\\
        
        \cline{1-4}
\hline

\hline

\hline

\hline
    \end{tabular}
  \caption{\textbf{Ablation on dual-criterion context selection. } Columns show model performance when using both sequence homology and text/QA similarity (Dual), sequence homology only (SeqOnly), or text/QA similarity only (QAOnly) to guide exemplar selection. Metric: ROUGE-L.
  }
    \label{tab:ablation}
\end{table}

==> table/retrieve_vs_random.tex <==
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{8pt}
\renewcommand\arraystretch{1.2}
    \centering\small
    \begin{tabular}{l|cc|c@{\hspace{8pt}}c@{\hspace{8pt}}|c@{\hspace{8pt}}c}
\hline

\hline

\hline

\hline
        \multirow{2}{*}{\bf Model}& \multicolumn{2}{c|}{\bf ProtDescribe} & \multicolumn{2}{c|}{ \bf Protein2Text-QA}&\multicolumn{2}{c}{\bf Mol-Instructions}  \\
         & Random & Retrieved & Random
 & Retrieved & Random & Retrieved \\ 
\hline
        Qwen2.5-3B~\cite{qwen2.5} & 23.60 & 27.32 & 20.09 & 28.66 & 19.77 & 21.35 \\
        Mistral-7B-Instruct-v0.3~\cite{chaplot2023albert} & 21.74 & 29.39 & 21.01 & 28.59 & 15.30 & 19.12\\
         Qwen3-14B~\cite{qwen3technicalreport} & 26.80 & 25.53 & 24.11 & 25.93 & 17.02 & 19.82\\
         kimi-k2~\cite{team2025kimi} & 30.23 & 35.91 & 20.48 & 21.04 & 13.75 & 15.54\\
         GPT-4o~\cite{openai2024gpt4} & 29.20 & 35.51 & 23.48 & 26.86 & 17.97 & 19.89\\
        
        \cline{1-4}
\hline

\hline

\hline

\hline
    \end{tabular}
  \caption{\textbf{Comparison of random and retrieved Example Selection. }Metric: ROUGE-L.
  }
    \label{tab:retrieve_vs_random}
\end{table}
